Visual Saliency Maps Can Apply to Facial Expression Recognition

Human eyes concentrate different facial regions during distinct cognitive activities. We study utilising facial visual saliency maps to classify different facial expressions into different emotions. Our results show that our novel method of merely using facial saliency maps can achieve a descent accuracy of 65\%, much higher than the chance level of $1/7$. Furthermore, our approach is of semi-supervision, i.e., our facial saliency maps are generated from a general saliency prediction algorithm that is not explicitly designed for face images. We also discovered that the classification accuracies of each emotional class using saliency maps demonstrate a strong positive correlation with the accuracies produced by face images. Our work implies that humans may look at different facial areas in order to perceive different emotions.

==> secs/discussion.tex <==
\section{Discussion}

\subsection{Estimating Our Proposed Model}

Given the transition and the emission matrices we generated for each representative model,
we can calculate the Viterbi path of the states the model would most likely go through. In this section, we will randomly pick some real eye movement sequence from our participants, and fit them into the obtained representative models and compute the percentage of the actual eye movement sequence that agrees with the likely states sequence. And we consider the model with the highest probability to be the cluster the eye movement sequence belongs to. To test the accuracy of the model classification, for each participant, we consider three typical eye
movement data that generate from conditions of telling-truth-on-familiar- faces, telling-truth- on-unfamiliar-faces, and lying-on-familiar-faces separately to be the testing set. The total number of the testing eye movement sequence is sixty-three.
17 out of 21 participants (i.e. 80.95\%) of telling-truth-on-familiar-face patterns are classified to correct cluster, 4 of the incorrect ones are classified to the telling-truth-on-unfamiliar faces.
13 out of 21 participants (i.e. 61.90\%) of telling-truth-on-unfamiliar-face patterns are
classified to correct cluster, 4 of the incorrect ones are classified to the lying-on-familiar-faces, 3 of the incorrect ones are classified to the telling-truth--on-familiar-faces.
17 out of 21 participants (i.e. 80.95\%) of lying-on-familiar-face patterns are classified to correct cluster, 2 of the incorrect ones are classified to the telling-truth-on-familiar-faces, 2 of the incorrect ones are classified to the telling-truth-on-unfamiliar-faces.
The accuracy of all the three circumstances are well above chance. The results show that the eye movement patterns when people are looking at familiar faces are consistent, as the accuracy of classification are both high in telling-truth-on-familiar-face and lying-on-familiar-face conditions. When people are looking at unfamiliar faces, the eye movement pattern is less consistent among different people but the accuracy is still close to double chance.

\subsection{Some Discussion}

We found that the general eye movement patterns in the condition of telling-truth-on-familiar- faces, telling-truth-on-unfamiliar-faces, and lying-on-familiar-faces has significant differences in not only the ROI location and area, but also the transition probabilities and time sequence of ROI.
When the participants are lying about their familiarity level of the viewed face, the ROIs tend to locate on the central axis of the face from top to bottom. When the participants are telling truth about the faces, the ROIs tend to locate at regions close to the two eyes and the region covers nose and mouth, which is an approximate triangle with its vertex composed by the three regions as described.
Differences between telling the truth about the familiarity level while viewing familiar and unfamiliar faces can be observed in the time order of the ROI sequence. Both of the eye movement patterns tend to start from the upper part of the face, while for the first situation, the scan path is most likely to start from the left eye from observer perspective, and for the second one, the initial fixation tend to locate at the right eye, again, from observer perspective. The most likely subsequent paths are also different, strategy for viewing familiar face is moving in between the two eye regions from observer perspective (remain or move back and forth); strategy for viewing unfamiliar face is moving in between the left eye region and the lower part of the face, still, from observer perspective (remain or move back and forth). Nevertheless, differences between the third case and the first two cases is quite obvious, however, it seems like that the general ROI of the first and second cases are similar (i.e. A general triangular path consisting of two eyes and the tip of the nose), and the range can not be a distinct characteristic to distinguish from each other.
In addition, during the real-world investigation, we can find the difference not only exists in time order of the states sequence from the transition probabilities, but also in the way fixations distribute. As can be seen from the Table 5.4 and 5.5, the representative ROI clustering centers of the first and second case are:
Case 1 (634.9725, 351.6586) (676.1114, 493.2836) (706.2081, 332.5524) Case 2 (672.2400, 430.2586) (616.2596, 321.0105) (688.8656, 337.2602) And the center of the face should be at (683, 384), by calculating the variance between the ROI clustering centers and the face center, the value of case 2 is significantly lower than the value of case 1, both on x and y dimension. Thus, we can infer that when people are viewing an unfamiliar face, the eye gaze can be more focused on the internal region of the face.

==> secs/experiments.tex <==
\section{Experiments}

\subsection{Face Image Preprocessing}

The variety of brightness and colors of photos can cause differences in human eye saccades and fixations, as well as a significant latency of the reaction time for viewing the same images~\cite{kalloniatis2007light}. We wish to minimize the noises resulting from this process, known as adaptation in ocular physiology. Therefore, we normalize all the experimental face images to be consistent with the same grey-scale and size of $447\times335$. Furthermore, we apply an oval mask to all the other parts of the images, including hairs, backgrounds and so on, except the main face area. This is to avoid the eye gaze being distracted by the background and objects other than our interested regions, namely human faces. One original face image and its processed result is as Figure \ref{fig:dean_and_masked}. 
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/dean_and_masked.png}
    \caption{One original face image and its processed result. }
    \label{fig:dean_and_masked}
\end{figure}

\subsection{Face Images and Participants}

We collected a total of 20 different gray-scale frontal-view face images, each will be displayed two times in a random order, one corresponding to telling the truth and the other for lying. That is, one participant will observe 40 images in total during the experiment. Among These faces, 15 out of 20 correspond to university lectures from two distinct faculties. Correspondingly, participants were sampled from these two faculties to ensure students from a particular faculty can recognize half of the lecture faces from their own faculty and have no knowledge for the rest half from the other one. The rest five were sourced from an online face database. In total, we recruited 21 participants. 

\subsection{Experimental Procedure}

We developed a web-browser based user interface to display our collected face images to the participants. During the experimental procedure, a participant will firstly see a huge instruction indicating either to ``tell the truth!'' or ``lie!'' for the upcoming face image. For example, if the face to display is familiar to the participant, he or she is expected to pretend to have no knowledge about the shown image. The same instruction will be prompted again to the participant before he or she gives the answer in order to avoid the unexpected honesty. We record participants' eye fixations trajectories during this process. Figure \ref{fig:ui_prompt} gives some screenshots of our user interface. 
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/ui_prompt.png}
    \caption{Screenshots of our user interface. }
    \label{fig:ui_prompt}
\end{figure}




==> secs/methods.tex <==
\section{Methods}

\subsection{Fixation Identification}

The raw eye gaze data is in the form of the Cartesian coordinate system, namely its locations are expressed by $(x, y)$ coordinates. It is essential to separating and labelling eye tracking points as fixations or saccades, since improper classification can have dramastic influence on higher-level analyses~\cite{salvucci2000identifying}. 

The dispersion threshold algorithm is considered to be the most robust and accurate approach for identifying fixations and saccades in eye-tracking protocals compared with other approaches such as velocity-based and area-based ones~\cite{salvucci2000identifying}. One essential parameter for this algorithm is called the pixel tolerance, which is a threshold that determines whether to classify a new eye-stare point as a fixation or a saccade. Previous research reported that a normal fixation duration is about 200-250 ms~\cite{miyao1989effects}, and each of our stimulus video lasts for five seconds. Thus, we can deduce that 20 fixation points per video should be an reasonable number, which leads to a setting of the pixel tolerance being 5. Figure \ref{fig:fixations_transition_paths} presents an example of the result using the dispersion threshold algorithm. 
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/fixations_transition_paths.png}
    \caption{Fixations and the transition paths (i.e. saccades) by using the dispersion threshold algorithm. Black dots are fixation points and blue lines represent eye saccade paths. }
    \label{fig:fixations_transition_paths}
\end{figure}

\subsection{Eye Movement Analysis}

\label{subsec:eye_movement_analysis}

We apply probabilistic graphical models, specifically Gaussian Hidden Markov models (HMMs with 2D Gaussian emission distribution), to train the previous collected eye movement data from participants. This technique is broadly utilized to model data generated from Markov processes~\cite{Bishop:2006:PRM:1162264, chuk2014understanding}. That is, the next state of a process only depends on its previous state. For every pair from a current state $S$ to its subsequent state $S'$ in the next time step, or to the observable state in the same time step $O$, there is an associated probability indicating the likelihood of transforming $S$ to $S'$ or $S$ to $O$, which can be formalized as a matrix. Finally, a vector of prior probabilities reveals the different probabilities of being on distinct starting states. We hypothesize to obtain different representative eye movement patterns during face recognition with distinct latent mental activities, namely telling the truth or lying. In this context, states represent different ROIs of a face image, observable states are fixation points, and the transition from the current latent state to the next state is a saccade. 

This methodology requires determining the number of facial regions of interests, i.e., Region of Interests (ROIs) beforehand. We pick the number as two and three. Picking three is since previous studies show that there are three information-rich inner regions of the face (eyes, nose, and mouth), which are particularly essential for person recognition~\cite{o2001familiarisation}. 

% Notwithstanding, for our last studied case, the extensive majority eye fixation points locate on the regions of two eyes. Thus, we choose the number of ROIs as two for that solely case. We will give more detailed explanation in Section \ref{sec:result}. 

In our case, we set the concentration parameters of Dirichlet prior distributions of initial distribution and transition probability to be 0.01. The prior covariance was set as an isotropic covariance matrix with standard deviation of 14 to ensure that the ROI has roughly the same size as the facial features. 

We first trained a Gaussian-HMM using the fixation data from one participant who was viewing images under a certain cognitive condition. For example, the participant has been instructed to tell the truth, followed by observing familiar faces. Fixation sequences during every observation is considered as viewing sequences. Followed by applying the Gaussian-HMM algorithm on multiple observation sequences, we can get a representative Gaussian-HMM with three states. Each state consists of three means and three covariance matrices representing the ROI centers and ranges. 

For every participant, there are four Gaussian-HMMs representing four different eye movement strategies, corresponding two degrees of face familiarity and lying or not. As a result, we have 84 Gaussian-HMMs from 21 participants, and classify them into four classes based on the face familiarity and lying cognitions. Afterwards, we train another Gaussian-HMM for each category in order to find a class representative Gaussian-HMM and its clustering centroids of its ROIs. Eventually, we will have four representative Gaussian-HMMs, each will contain its clustering centroids of ROIs, shapes of ROIs, an intial distribution vector of ROIs, a transition probability matrix, and a Viterbi path. 


